Crop mapping from image time series: deep learning with multi-scale label hierarchies

The aim of this paper is to map agricultural crops by classifying satellite image time series. Domain experts in agriculture work with crop type labels that are organised in a hierarchical tree structure, where coarse classes (like orchards) are subdivided into finer ones (like apples, pears, vines, etc.). We develop a crop classification method that exploits this expert knowledge and significantly improves the mapping of rare crop types. The three-level label hierarchy is encoded in a convolutional, recurrent neural network (convRNN), such that for each pixel the model predicts three labels at different level of granularity. This end-to-end trainable, hierarchical network architecture allows the model to learn joint feature representations of rare classes (e.g., apples, pears) at a coarser level (e.g., orchard), thereby boosting classification performance at the fine-grained level. Additionally, labelling at different granularity also makes it possible to adjust the output according to the classification scores; as coarser labels with high confidence are sometimes more useful for agricultural practice than fine-grained but very uncertain labels. We validate the proposed method on a new, large dataset that we make public. ZueriCrop covers an area of 50 km x 48 km in the Swiss cantons of Zurich and Thurgau with a total of 116'000 individual fields spanning 48 crop classes, and 28,000 (multi-temporal) image patches from Sentinel-2. We compare our proposed hierarchical convRNN model with several baselines, including methods designed for imbalanced class distributions. The hierarchical approach performs superior by at least 9.9 percentage points in F1-score.

==> 09_limitation.tex <==
\textcolor{blue}{
\section{Limitations \& Future Work}
\label{limitations}
%
There are few limitations of the proposed approach that we briefly discuss them and to address those limitations we leave some ideas to be explored in future work for the interested reader.
%
(i) Like many deep networks the current model requires a significant amount of training labels for best performance. It would be interesting to improve the sample efficiency, perhaps with active learning schemes, as a large set of reference data may not be always be available.
%
(ii) Also data-driven models, like the one proposed in this paper, are intrinsically tied to the data used during training. A domain shift e.g caused by a change in target crop types or change in weather conditions, which influences appearance of vegetation, would necessarily require a re-training or fine-tuning of the model for similar performance requirements. 
Pairing our method with a meta-learning scheme, e.g., one explored in \citep{russwurm2020meta}, could ease the adaptation of our model to different crop types and different geographic regions. 
%
(iii) The label hierarchy in this work is specific to Switzerland, different hierarchies may be needed for other geographic regions. %
In that context it should be noted that hard-coding a particular label hierarchy into the network architecture is an inherent part of the current design, but lacks flexibility when moving to other environments. A technically challenging, but potentially useful extension to current method could be to learn the label hierarchy from data rather than impose it a-priori, for instance with unsupervised learning techniques or interleaved with the classifier training.}


%Moreover, the detection still fails almost entirely for a number of extremely rare crops. At this point it remains unclear whether this behaviour can be addressed with current machine learning technology, and where the limits are in terms of rarity and imbalance. 

%add subsection 6.6 on the limitations of the proposed approach (including those what you answered to me). For example, you mentioned "Data driven models, like the one proposed in this paper, are intrinsically tied to the data used during training. A domain shift would necessarily require a re-training or ne-tuning of the model."

%with clear discussions on the data quality issues/limitations and considerations.

%Please add discussion that the authors are not sure on how the method will be applied to other areas with more cloud and more filled pixels.



%Maximising data efficiency was not the focus of this work, still we provide the requested results to show how the amount of available reference labels affects model performance. As suggested by the AE, we have trained the model on one and two stripes, which roughly correspond to 20\% and 40\% of the total labels. Results are shown in Table~\ref{table:small_set}. As expected, fewer labels cause a gradual performance drop that most strongly affects the rare classes (hence overall accuracy  remains fairly high). 

%To adequately capture the characteristic features of rarer classes with comparatively few labels, it seems entirely possible to pair our model with an \emph{active learning} scheme. However, this would constitute a project on its own and goes beyond the scope of this study.\\


%Future work
%There are several interesting options for future work to extend the proposed method and to address its current limitations.

